Programming Language Agnostic Mining of Code and Language Pairs with Sequence Labeling Based Question Answering

Mining aligned natural language (NL) and programming language (PL) pairs is a critical task to NL-PL understanding. Existing methods applied specialized hand-crafted features or separately-trained models for each PL. However, they usually suffered from low transferability across multiple PLs, especially for niche PLs with less annotated data. Fortunately, a Stack Overflow answer post is essentially a sequence of text and code blocks and its global textual context can provide PL-agnostic supplementary information. In this paper, we propose a Sequence Labeling based Question Answering (SLQA) method to mine NL-PL pairs in a PL-agnostic manner. In particular, we propose to apply the BIO tagging scheme instead of the conventional binary scheme to mine the code solutions which are often composed of multiple blocks of a post. Experiments on current single-PL single-block benchmarks and a manually-labeled cross-PL multi-block benchmark prove the effectiveness and transferability of SLQA. We further present a parallel NL-PL corpus named Lang2Code automatically mined with SLQA, which contains about 1.4M pairs on 6 PLs. Under statistical analysis and downstream evaluation, we demonstrate that Lang2Code is a large-scale high-quality data resource for further NL-PL research.

==> contents/downstream.tex <==
% \section{Downstream Evaluation}


% % Description of the experiments
% \subsection{Experiments}
% Xu et. al \cite{incorporating_conala} used a transition based LSTM model tranX, to show the effectiveness of combining multiple data sources. They first pretrained the model on 100k auto-mined CoNaLa data, then fine tuned on CoNaLa-human training set, and then evaluated on the CoNaLa-human test set. We reproduced their experiments with publicly available code, and then conducted a series of additional experiments replacing the CoNaLa-mined data with Lang2Code data.

% \subsection{Baseline}

% \begin{itemize}
% [topsep=0.2em]
%     \setlength\itemsep{-.2em}
%     \item {\textbf{Man} refers to trained solely on CoNaLa-human training set.}
%     \item {\textbf{Man+CoNaLa-Mined 100k} denotes the model first pretrained with top 100k CoNaLa-mined NL-PL pairs, and then fine-tuned with CoNaLa-man}
%     \item {\textbf{Man+Lang2Code-Mined 100k} first pretrained the model on top 100k Lang2Code-mined and then fine-tuned on CoNaLa training set.}
%     \item {\textbf{Man+Lang2Code-Mined 100k clean} To better approximate the distribution of the CoNaLa dataset, we simply removed code snippets longer than 100 characters, and removed the import statements, as they are considered by CoNaLa as contexts rather than code snippets. 
%     After that, we first pretrained the model on top 100k cleaned Lang2Code-mined NL-PL pairs, and then fine-tuned on CoNaLa training set.}
%     \item {\textbf{Man+Lang2Code-Mined all clean} we first pretrained the model on all cleaned Lang2Code-mined NL-PL pairs, which is around 200k, and then fine-tuned on CoNaLa training set.}    
    
% \end{itemize}

% Man refers to trained solely on CoNaLa-human training set.

% Man+CoNaLa-Mined denotes the model first pretrained with CoNaLa-mined and then fine-tuned with CoNaLa-man

% Man + Lang2Code-Mined first pretrains the model on Lang2Code-mined and then fine-tuned on CoNaLa training set.





% We select the top 100k Lang2Code-mined using the confidence score, to have the same number of pairs with the CoNaLa-mined experiments.

% % This line if the 100k-short experiments succeeded
% We removed all the import statements and filtered out code snippets longer than 100 tokens, to make the data distribution closer to CoNaLa, as later is a sub code block level datasets.

% \subsubsection{Results}









